Motivational models for validating agile requirements in Software Engineering subjects

This paper describes how motivational models can be used to cross check agile requirements artifacts to improve consistency and completeness of software requirements. Motivational models provide a high level understanding of the purposes of a software system. They complement personas and user stories which focus more on user needs rather than on system features. We present an exploratory case study sought to understand how software engineering students could use motivational models to create better requirements artifacts so they are understandable to non-technical users, easily understood by developers, and are consistent with each other. Nine consistency principles were created as an outcome of our study and are now successfully adopted by software engineering students at the University of Melbourne to ensure consistency between motivational models, personas, and user stories in requirements engineering.

==> references.tex <==
@book{sterling2009art,
  title={The art of agent-oriented modeling},
  author={Sterling, Leon and Taveter, Kuldar},
  year={2009},
  publisher={MIT Press}
}
@incollection{quitch,
  title={Using Motivational Modelling with an App Designed to Increase Student Performance and Retention},
  author={Sterling, Leon and Pedell, Sonja and Oates, Grainne},
  booktitle={Early-Warning Systems and Targeted Interventions for Student Success in Online Courses},
  pages={161--176},
  year={2020},
  publisher={IGI Global}
}
@incollection{Sterling2018EmergencyAlarms,
    title = {Adding emotions to models in a viewpoint modelling framework from agent-oriented software engineering: A case study with emergency alarms},
    year = {2018},
    booktitle = {Innovative Methods, User-Friendly Tools, Coding, and Design Approaches in People-Oriented Programming},
    author = {Sterling, Leon and Lopez-Lorca, Alex and Kissoon-Curumsing, Maheswaree},
    isbn = {9781522559702},
    doi = {10.4018/978-1-5225-5969-6.ch010}
}

@INPROCEEDINGS{Lopez-Lorca,
 author = {Lopez-Lorca, Antonio and Burrows, Rachel and Sterling, Leon},
  title = {Teaching Motivational Models in Agile Requirements Engineering},
  booktitle = {Proceedings of the Requirements in Education and Training workshop
    at RE'18},
  year = {2018},
  location = {Banff, Canada}
 }
@incollection{marshall2018agent,
  title={Agent-based modelling of emotional goals in digital media design projects},
  author={Marshall, James},
  booktitle={Innovative Methods, User-Friendly Tools, Coding, and Design Approaches in People-Oriented Programming},
  pages={262--284},
  year={2018},
  publisher={IGI Global}
}

@incollection{ontology-validation,
  title={Ontology-mediated validation of software models},
  author={Lopez-Lorca, Antonio A and Beydoun, Ghassan and Sterling, Leon and Miller, Tim},
  booktitle={Information Systems Development},
  pages={455--467},
  year={2011},
  publisher={Springer}
}

@article{inayat2015systematic,
  title={A systematic literature review on agile requirements engineering practices and challenges},
  author={Inayat, Irum and Salim, Siti Salwah and Marczak, Sabrina and Daneva, Maya and Shamshirband, Shahaboddin},
  journal={Computers in human behavior},
  volume={51},
  pages={915--929},
  year={2015},
  publisher={Elsevier}
}
@article{beck2001manifesto,
  title={Manifesto for agile software development},
  author={Beck, Kent and Beedle, Mike and Van Bennekum, Arie and Cockburn, Alistair and Cunningham, Ward and Fowler, Martin and Grenning, James and Highsmith, Jim and Hunt, Andrew and Jeffries, Ron and others},
  year={2001}
}

@article{bhat2006overcoming,
  title={Overcoming requirements engineering challenges: Lessons from offshore outsourcing},
  author={Bhat, Jyoti M and Gupta, Mayank and Murthy, Santhosh N},
  journal={IEEE software},
  volume={23},
  number={5},
  pages={38--44},
  year={2006},
  publisher={IEEE}
}
@article{schon2017agile,
  title={Agile Requirements Engineering: A systematic literature review},
  author={Schon, Eva-Maria and Thomaschewski, Jorg and Escalona, Maria Jose},
  journal={Computer Standards \& Interfaces},
  volume={49},
  pages={79--91},
  year={2017},
  publisher={Elsevier}
}
@article{cao2008agile,
  title={Agile requirements engineering practices: An empirical study},
  author={Cao, Lan and Ramesh, Balasubramaniam},
  journal={IEEE software},
  volume={25},
  number={1},
  pages={60--67},
  year={2008},
  publisher={IEEE}
}
@article{daneva2013agile,
  title={Agile requirements prioritization in large-scale outsourced system projects: An empirical study},
  author={Daneva, Maya and Van Der Veen, Egbert and Amrit, Chintan and Ghaisas, Smita and Sikkel, Klaas and Kumar, Ramesh and Ajmeri, Nirav and Ramteerthkar, Uday and Wieringa, Roel},
  journal={Journal of systems and software},
  volume={86},
  number={5},
  pages={1333--1353},
  year={2013},
  publisher={Elsevier}
}
@inproceedings{bjarnason2011case,
  title={A case study on benefits and side-effects of agile practices in large-scale requirements engineering},
  author={Bjarnason, Elizabeth and Wnuk, Krzysztof and Regnell, Bj{\"o}rn},
  booktitle={proceedings of the 1st workshop on agile requirements engineering},
  pages={1--5},
  year={2011}
}
@inproceedings{blomkvist2015communication,
  title={Communication through boundary objects in distributed agile teams},
  author={Blomkvist, Johan Kaj and Persson, Johan and {\AA}berg, Johan},
  booktitle={Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems},
  pages={1875--1884},
  year={2015}
}
@inproceedings{dittmar2019integrating,
  title={Integrating personas and use case models},
  author={Dittmar, Anke and Forbrig, Peter},
  booktitle={IFIP Conference on Human-Computer Interaction},
  pages={666--686},
  year={2019},
  organization={Springer}
}
@inproceedings{faily2013guidelines,
  title={Guidelines for integrating personas into software engineering tools},
  author={Faily, Shamal and Lyle, John},
  booktitle={Proceedings of the 5th ACM SIGCHI symposium on Engineering interactive computing systems},
  pages={69--74},
  year={2013}
}

@inproceedings{schneidewind2012personas,
  title={How personas support requirements engineering},
  author={Schneidewind, Lydia and H{\"o}rold, Stephan and Mayas, Cindy and Kr{\"o}mker, Heidi and Falke, Sascha and Pucklitsch, Tony},
  booktitle={2012 First International Workshop on Usability and Accessibility Focused Requirements Engineering (UsARE)},
  pages={1--5},
  year={2012},
  organization={IEEE}
}

@inproceedings{ferreira2015designing,
  title={Designing Personas with Empathy Map.},
  author={Ferreira, Bruna and Silva, Williamson and Oliveira, Edson and Conte, Tayana},
  booktitle={SEKE},
  volume={152},
  year={2015}
}

@inproceedings{kamthan2015using,
  title={Using Personas to Support the Goals in User Stories},
  author={Kamthan, Pankaj},
  booktitle={2015 12th International Conference on Information Technology-New Generations},
  pages={770--770},
  year={2015},
  organization={IEEE}
}

@inproceedings{castro2008integrating,
  title={Integrating the personas technique into the requirements analysis activity},
  author={Castro, John W and Acu{\~n}a, Silvia T and Juristo, Natalia},
  booktitle={2008 Mexican International Conference on Computer Science},
  pages={104--112},
  year={2008},
  organization={IEEE}
}
@book{cohn2004user,
  title={User stories applied: For agile software development},
  author={Cohn, Mike},
  year={2004},
  publisher={Addison-Wesley Professional}
}
